NetDiffus: Network Traffic Generation by Diffusion Models through Time-Series Imaging

Network data analytics are now at the core of almost every networking solution. Nonetheless, limited access to networking data has been an enduring challenge due to many reasons including complexity of modern networks, commercial sensitivity, privacy and regulatory constraints. In this work, we explore how to leverage recent advancements in Diffusion Models (DM) to generate synthetic network traffic data. We develop an end-to-end framework - NetDiffus that first converts one-dimensional time-series network traffic into two-dimensional images, and then synthesizes representative images for the original data. We demonstrate that NetDiffus outperforms the state-of-the-art traffic generation methods based on Generative Adversarial Networks (GANs) by providing 66.4% increase in fidelity of the generated data and 18.1% increase in downstream machine learning tasks. We evaluate NetDiffus on seven diverse traffic traces and show that utilizing synthetic data significantly improves traffic fingerprinting, anomaly detection and traffic classification.

==> 02_Intro.tex <==
\section{Introduction}

Global network traffic has ever been increasing during the past two decades making it difficult for network operators to smoothly continue their operations. For example, with the sheer volume of network transactions, many tools equipped  with in-network packet analysis such as middleboxes for traffic analytics, systems for intrusion detection, and traffic policing systems are struggling to provide better service\revise{~\cite{}}. This situation has been overwhelmed by end-to-end encryption causing deep packet inspection based approaches ineffective in scenarios such as anomaly detection~\cite{kattadige2021360norvic}.

To this end, Machine Learning (ML) based solutions have been proposed over the first few years which have created significant improvements in network traffic analytics~\revise{\cite{kattadige2021360norvic,dimopoulos2016measuring,xie2018survey,du2020machine}}. Generally, these ML models require a large number of data to train the models to achieve highly accurate results during inference phases. Moreover, these training samples should adequately represent all possible variations of the data to make the trained model robust. However, collecting useful traffic data from real networks is challenging due to multiple reasons.

First, modern network systems are highly complex. Hence, deploying data collection tools in these complex settings is really challenging which is further exacerbated by the sheer volume of network data transferred through them~\revise{\cite{kattadige2021seta++, sperotto2010overview}}. This situation has often made it difficult for filtering out the required traffic data further affecting its purity. Second, collecting network traffic from real users can raise many legal and ethical issues particularly related to the privacy of the users~\revise{\cite{sun2020iot}}. Third, many organizations are reluctant to share the real data collected with others, even maybe with different departments of the same organization, due to policy and regulation constraints~\revise{\cite{lin2020using}}. 

To overcome these issues, synthetic data generation has become a promising approach. In these approaches, generative models (e.g., GANs--Generative Adversarial Models, Diffusion models (DM)) are trained using a known set of data, which can be limited in amount, and the trained model synthesize unseen data that are not identical to the actual data but have the same properties. Though, generative models have been widely applied in image, audio and text generation, a very limited amount of work has been done in network traffic generation. As collecting real network data with high purity is extremely challenging, synthetic data generation for network traffic is indispensable to support downstream network analysis tasks, particularly with ML models. 

As a solution, in \solution{} (\textbf{Net}work Traffic Generation by \textbf{Diffus}ion Models through Time-Series Imaging), we present synthetic data generation for network traffic data leveraging recently proposed diffusion model (DM) architectures. DM has shown outstanding performance compared to  other state-of-the-art generative models such as GANs in different domains and data types. Observing the improved generation performance for 2D data and the higher accuracy in downstream ML tasks, we first convert 1D network traffic traces into a special image format called GASF (Grammian Angular Summation Field)~\revise{\cite{wang2015imaging,barra2020deep,dias2019image,qin2020imaging}}. Then, we take these images to train a standard DM, which synthesize data in the same image format. We leverage these synthetic data to show improved accuracy in downstream  ML tasks related to network.  

% We use over ------ actual network traces (i.e., sequence of packet traces) to generate over ----- synthetic traces representing three major traffic 

To the best of our knowledge, this is the first attempt at utilizing standard DM for network data generation.  Contributions of \solution{} are mainly four folds. First, We show a standard DM model is sufficient to synthesize network traffic data with high fidelity by converting time-series to GASF image format. Second, we leverage three different network traffic types: video, web (i.e., accessing web pages) and IoT, representing the majority contributors of  the global network traffic~\revise{\cite{}}. Third, we apply generated synthetic traces for three main network related use cases and show a wide range of accuracy improvements (1-57\%) in ML tasks, especially including critical data-limited scenarios. Finally, we show that \solution{} can outperform state-of-the-art GAN based models and 1D synthetic data from corresponding 1D DMs. Artificats of \solution{} -- \textit{are hidden for double blind review --}.






==> 04_Background_motivation.tex <==
\section{Background and motivation}

\subsection{Improvement in ML by imaging network traces}\label{subsec:improvement ml image}

We first analyzed the performance gain  by converting 1D network traces into 2D images in ML based classification tasks. For this analysis, we select video fingerprinting related ML task from~\cite{madarasingha2022videotrain++} and its related 1D trace dataset, which we denote as \textbf{D1} in Section~\ref{subsec:dataset}). We leverage GASF images as the 2D format\cite{wang2015imaging,dias2019image, barra2020deep, qin2020imaging}. 
First, we convert the 1D time series to GASF image format followed by feeding them for ML based classification. For the 1D-trace based evaluation, we use NN model from~\cite{madarasingha2022videotrain++} with 1D convolution. We use the same model for GASF image classification, substituting 1D convolutions with 2D convolutions. 
In brief, ML classifier tries to classify a given test video trace from  a content platform (e.g., YouTube, Netflix or Stan) to one of the 20  videos (i.e., classes). The models are trained with traces from the same video classes. None of the train traces appear in test sets. We vary the train set size as 80, 40 and 20\% of the original dataset and always keep the last 20\% as the test set.

From Table~\ref{table: 1D classification vs 2D classification}, we observe that GASF images achieve 6.7\% of average accuracy increase across all scenarios having 13.3\% of maximum for \textbf{D1-Netflix}. The main reason for accuracy gain is GASF images additionally map the correlations between 1D trace sample points onto one image making it a rich source of information compared to longer 1D sequences. This has revealed the effectiveness of conversion of 1D traces to 2D GASF images in network traffic related ML tasks. Empirically observed that compared to other similar image formats such as GADF and MTF, GASF achieves higher accuracy and preserves the bijective property (i.e., reconstruct 1D traces from GASF images). This further verified the suitability of GASF images for \solution{}.

\begin{table}[h]
    \centering
    % \captionsetup{justification=centering}
    \small{
    \caption{Accuracy (\%) of a video fingerprinting classification for different percentages of original data.
    1D (time series trace) vs 2D (GASF images)}
    \vspace{-2mm}
    \label{table: 1D classification vs 2D classification}
    \begin{tabular}{lcccccc}

        \toprule
        {Platform} &
            \multicolumn{2}{c}{80\% data} &
            \multicolumn{2}{c}{40\% data} &
            \multicolumn{2}{c}{20\% data} \\
            \textbf{D1-} & 1D & 2D & 1D & 2D & 1D & 2D \\
             
        \midrule
        
        \textbf{YT}  & 90.5 & \textbf{92.5} & 85.5 & \textbf{87.0} & 71.0 & \textbf{75.0}  \\
        \textbf{Stan}  & 91.0 & \textbf{99.0} & 96.0 & \textbf{98.0} & 90.0 & \textbf{93.0}\\
        \textbf{Netflix}  & 83.0 & \textbf{100.0} & 84.0 & \textbf{97.0} & 78.0 & \textbf{88.0}  \\
        \bottomrule
    \end{tabular}
    }
\end{table}





% removed the content for CONext by moving part of the content to the Section 3.1
% \subsubsection{Why we selected GASF format?} We further compare the GASF images with different other imaging formats, GADF and MTF from the literature~\cite{wang2015imaging} by running the same ML classification in Section~\ref{subsec:improvement ml image} for YT and Stan datasets. First, we observe that compared with the other two formats, GASF images provide higher classification performance. For example, in YT, GASF images achieve over 3\% and 81\% accuracy 81\% accuracy improvement compared to its GADF and MTF counterparts respectively and we notice the same trend for Stan dataset. Second, only GASF holds the invertibility property which is essential for the 1D domain analysis after converting synthetic 2D images to corresponding 1D traces. Based on these facts, we select GASF as our format for further experiments.










% Table~\ref{table:compare diff image format} reports the classification accuracy for \textbf{D1-YT} and \textbf{D1-Stan} along with its  invertibility property (i.e., ability to re-construct 1D traces from 2D images). We see that compared to the other two image formats, GASF images provide higher classification performance. For example, \textbf{D1-YT} GASF images achieve over 3\% and 


% \begin{table}[h]
    
%     \centering
%     \caption{{Comparison with different image formats}}
%     \vspace{-1mm}
%     \label{table:compare diff image format}
%     \small
%     \begin{tabular}{llrr}
%         \toprule
%         {Image (type)} & {Dataset}  & {Classifier Per.}    & {Invertible}\\
%           & & {Accuracy(\%)} & \\
%         \midrule
%        {GASF} &\textbf{{D1-YT}}    & {92.5}     &{Yes} \\
%          &\textbf{{D1-Stan}} & {99.0}    & {Yes}\\
%         \midrule
%         {GADF} &\textbf{{D1-YT}}    & {91.0}      & {No} \\
%          &\textbf{{D1-Stan}} & {96.0} & {No}  \\
%          \midrule
%          {MTF} &\textbf{{D1-YT}}    & {57.0}   &{No} \\
%          &\textbf{{D1-Stan}} & {18.0}   & {No}\\
         
%         \bottomrule
%     \end{tabular}
% \end{table}



% \subsection{Converting 1D traces to 2D GASF images}\label{subsec:gasf conversion}
\begin{figure}[h]
% % \vspace{-2mm}
    \centering
    \includegraphics[width=\columnwidth]{Figures/BG-motivation/1D_to_GASF_conversion_revised.pdf} 
    \caption{Conversion process: 1D traces to 2D GASF images.}
    \label{fig:gasf conversion}
\end{figure}

\subsection{GASF conversion and its properties}\label{subsec:gasf conversion}
Given a 1D signal, which  can be a time series distribution of a given network trace feature (e.g., bytes dl), we first convert it to polar coordinates followed by creating the corresponding Grammian matrix. Here, elements of the Grammian matrix denote the inner product between the cosine angles of the time series in the polar coordinate system, which is the base of the GAF (Grammian Angular Field). Also, by taking the inner product between different sample points, the matrix further represents a correlation map between the sample points in the 1D trace~\revise{\cite{wang2015imaging}}. Then we create  the GASF (i.e., GASF images) by taking the summation of  all the  pairs of elements in row and column directions. This process removes the dependency on the radius in the GAF data. Fig.~\ref{fig:gasf conversion} shows a sample GASF image in which each row and column indices of the image represent correlations between time points of the 1D trace.



% To further explain, as the Gramian matrix is created by taking the inner product between the cosine angles of the time series in the polar coordinate system, it creates a correlation between the sample points in the process.
% The elements of the Gramian matrix is the inner product between the cosine angles of different points of the time series in polar coordinate system which gives us the advantage of storing the correlation between any two points in the time series.
% for a given row ($u$: 1D sample point 1), columns($v$: 1D sample point 2) on a GASF image and time interval between two samples  is $\Delta$, $GASF_{u,v:|u-v|=\Delta}$ indicates the relative correlation by summation of directions w.r.t. $\Delta$\revise{\cite{}}.
% The elements of the Gramian matrix is the inner product between the cosine angles of different points of the time series in polar coordinate system which gives us the advantage of storing the correlation between any two points in the time series.
Appendix~\ref{append:gasf conversion} contains the detailed conversion process.

Compared to traditional images, we identify three main properties unique to GASF images, \textit{i})~The main diagonal represents the initial angular value, which can be used to reconstruct the original 1D trace\revise{~\cite{wang2015imaging}}, \textit{ii})~Image is symmetric around the main diagonal and \textit{iii})~Correlation values are distributed as noticeable vertical or horizontal strips when there are noticeable peaks in 1D traces. These properties distinguish GASF images from traditional images. 










==> 05_1_Datasets.tex <==
\subsection{Dataset}\label{subsec:dataset}

\begin{table}[h]
    \vspace{-2mm}
    \small
    \centering
    \caption{Summary of Datasets}
    \vspace{-2mm}
    \label{table:dataset}
    \begin{tabular}{llll}
        \toprule
        Dataset     & No. of    & Traces     & Downstream \\
                    & classes   & per class   & ML task\\
        \midrule
        \textbf{D1-YouTube}~\cite{kwon20208Seta} & 20    & 100 & \\
        \textbf{D1-Stan}    & 20    & 100 & video fingerprinting \\
        \textbf{D1-Netflix} & 20    & 100  & \\
        \midrule
        \textbf{D2-DF}~\cite{sirinam2018deep} & 20    & 900 & web fingerprinting \\
        \midrule
        \textbf{D3-Google}~\cite{choi2020passive}  & 10    & 1000  & IoT smart home  \\
        \textbf{D3-Alexa}   & 10    & 1000  & activity recognition\\
        
        \bottomrule
    \end{tabular}
\end{table}

In \solution{}, we leverage three main datasets, reported in Table~\ref{table:dataset}, representing three different network traffic. First, dataset 1 (\textbf{D1}) is related to video streaming sessions\footnote{A session represents streaming a given video for a given time period.} from three content providers YouTube, Stan and Netflix. From each platform, there are 20 classes and in each class, there are 100 traces. Here, a trace represents a time series distribution of bytes downloaded (dl) values.
% For this dataset, we have selected Bytes dl distribution which can substantially represent the properties in video streaming sessions. 
The intended ML task is to fingerprint a given trace by classifying it to one of the 20 videos of a given platform. 
% Fig.~\ref{fig:D1-YT}-(left) shows a sample trace from \textbf{D1-YT} dataset showing the periodic data transmission, which is common in most of the video streaming task, mainly due to the adaptive bit rate controlling algorithm in proprietary applications~\cite{kattadige2021360norvic}.
The dataset 2 (\textbf{D2-DF}) consists of web surfing traffic to a closed set of 20 websites from~\cite{sirinam2018deep}. The extracted feature is packet direction: (+1) for uplink and (-1) for downlink packets. 
% Fig.~\ref{fig:D2-cls}-(left) illustrates such packet direction distribution as time-series for  a randomly selected trace from \textbf{D2-DF}-Class 1. 
Each traffic trace is classified into one of the 20 classes (i.e., website) as
a website fingerprinting task. The dataset 3 by~\cite{choi2020passive} (\textbf{D3}) consists of IoT packet level traces collected when invoking 10 activities by \textit{Google Home} and \textit{Amazon Echo} devices. Captured traces represents the communication between the device and its corresponding server. 
% Each trace has packet direction and the size as shown in  Fig.~\ref{fig:D3-iot}-(left) for \textbf{D3-Google}-Class 1. 
Appendix~\ref{append:dataset-1d-gasf} illustrates randomly selected traces from each dataset and their corresponding GASF conversions.






==> 07_Results.tex <==
\section{Results}
\subsection{Fidelity of synthetic data}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{.48\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Results/Fidelity_experiments/cdf_fid_all.pdf}
        \caption{}
        \label{fig:fidelity fid}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.48\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Results/Fidelity_experiments/cdf_ssim_max.pdf}
        \caption{}
        \label{fig:fidelity ssim}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.48\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Results/Fidelity_experiments/cdf_rmse_min.pdf}
        \caption{}
        \label{fig:fidelity rmse}
    \end{subfigure}
    \hfill
    \begin{subfigure}{.48\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/Results/Fidelity_experiments/cdf_uqi_max.pdf}
        \caption{}
        \label{fig:fidelity uqi}
    \end{subfigure}
    
\caption{Fidelity distribution of 6 datasets in terms of FID, SSIM, RMSE and UQI values}
\label{fig:fidelity}
\end{figure*}

Fig. \ref{fig:fidelity} shows how the 4 metrics FID, SSIM, RMSE and UQI vary for the 6 datasets. 

\begin{figure}[h]
\centering
\begin{subfigure}{.5\columnwidth}
  \centering
  \includegraphics[width=.9\linewidth]{Figures/Results/Accuracy/ResAcc_vs_Synth_CSIRO.pdf}
  \caption{CSIRO dataset}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\columnwidth}
  \centering
  \includegraphics[width=.9\linewidth]{Figures/Results/Accuracy/ResAcc_vs_Synth_GoogleIoT.pdf}
  \caption{IoT dataset}
  \label{fig:sub2}
\end{subfigure}
\caption{Classifier accuracy vs number of synthasized samples}
\label{fig:test}
\end{figure}

==> 09_Conclusion.tex <==



% Data generation process consisted of data pre \& post-processing steps and the synthetic data were used to improve the performance in multiple network related ML tasks including surveillance through traffic fingerprinting, anomaly detection and near real-time predictions. While further analyzing different aspects of data synthesis such as impact of number of original traces for DM, comparison with corresponding 1D generation, we showed that \solution{} surpassed many state-of-the-art network traffic generation model, particular based on GAN.

% --- Will be moved to Discussion section ---
% In future works, we aim to apply stable diffusion model to further reduce the memory and processing overhead incurred by imaging time series to GASF format. Furthermore, we plan to extend our dataset for different network traffic and features to further generalize the \solution{}. 

